Forecasting Future Videos from Novel Views via Disentangled 3D Scene Representation

Video extrapolation in space and time (VEST) enables viewers to forecast a 3D scene into the future and view it from novel viewpoints. Recent methods propose to learn an entangled representation, aiming to model layered scene geometry, motion forecasting and novel view synthesis together, while assuming simplified affine motion and homography-based warping at each scene layer, leading to inaccurate video extrapolation. Instead of entangled scene representation and rendering, our approach chooses to disentangle scene geometry from scene motion, via lifting the 2D scene to 3D point clouds, which enables high quality rendering of future videos from novel views. To model future 3D scene motion, we propose a disentangled two-stage approach that initially forecasts ego-motion and subsequently the residual motion of dynamic objects (e.g., cars, people). This approach ensures more precise motion predictions by reducing inaccuracies from entanglement of ego-motion with dynamic object motion, where better ego-motion forecasting could significantly enhance the visual outcomes. Extensive experimental analysis on two urban scene datasets demonstrate superior performance of our proposed method in comparison to strong baselines.

==> sec/4_implementation_details.tex <==

%Models are trained on resolutions of $256 \times 832$ for KITTI \cite{geiger2013vision} and $512 \times 1024$ for Cityscapes \cite{geiger2013vision}.



==> sec/L_algo.tex <==
\section{Methodology}

\subsection{Step 1: Initial Frame Input}
We begin by taking two consecutive frames from a video sequence, denoted as $I_{(t-1)}$ and $I_{(t)}$, as input. These frames represent the visual data at two adjacent time points.

\subsection{Step 2: Depth Estimation}
Utilizing the depth estimation algorithm Zoedepth, we estimate the depth for both input frames. The resulting depth maps are denoted as $D_{(t-1)}$ and $D_{(t)}$, corresponding to each frame, respectively.

\subsection{Step 3: Semantic Segmentation for Segmenting Static Category Objects}
Each RGB input frame ($I_{(t-1)}$ and $I_{(t)}$) undergoes semantic segmentation to generate binary masks ($M_{(t-1)}$ and $M_{(t)}$). These masks distinguish static categories (e.g., buildings, roads, sidewalks, poles, vegetation) from dynamic categories (e.g., cars, buses, pedestrians). We refer to all the regions in the input image that belong to static categories as background and refer to all the regions in the input corresponding to dynamic categories to foreground. Note that binary masks ($M_{(t-1)}$ and $M_{(t)}$) identify the background regions of the corresponding images. Please check supplementary material for detailed description of categories.

\subsection{Step 4: Inpainting for Foreground Region Exclusion}
With the binary masks ($M_{(t-1)}$ and $M_{(t)}$) identifying background regions, we inpaint both the RGB frames and their corresponding depth maps to exclude the foreground (\ie dynamic) objects. The inpainted RGB frames are denoted as $I_{(t-1)}^{\text{inpaint}}$ and $I_{(t)}^{\text{inpaint}}$, and the depth maps as $D_{(t-1)}^{\text{inpaint}}$ and $D_{(t)}^{\text{inpaint}}$.

\subsection{Step 5: Feature Encoding }
The original and inpainted RGB frames ($I_{(t-1)}$, $I_{(t)}$, $I_{(t-1)}^{\text{inpaint}}$, and $I_{(t)}^{\text{inpaint}}$) are passed through a feature encoder to extract features. The features for the original frames are denoted as $F_{(t-1)}$ and $F_{(t)}$, and for the inpainted frames, we obtain $F_{(t-1)}^{\text{inpaint}}$ and $F_{(t)}^{\text{inpaint}}$.

\subsection{Step 6: Ego-Motion Forecasting}
For predicting ego-motion, we input the inpainted features ($F_{(t-1)}^{\text{inpaint}}$ and $F_{(t)}^{\text{inpaint}}$) and binary masks ($M_{(t-1)}$ and $M_{(t)}$) into an ego-motion forecasting neural network. This process yields the transformations $T_{(t-1) \rightarrow (t+1)}$ and $T_{(t) \rightarrow (t+1)}$, indicating the predicted ego-motion between frames.

\subsection{Step 7: Foreground Motion Prediction}
To forecast the motion of dynamic objects, the original features ($F_{(t-1)}$ and $F_{(t)}$) and binary masks ($M_{(t-1)}$ and $M_{(t)}$) are input into a foreground motion forecasting neural network. This yields 3D motion flows $u_{(t-1) \rightarrow (t+1)}$ and $u_{(t) \rightarrow (t+1)}$, representing the all the input regions across frames.

\section{Conclusion}
Your conclusion here.

==> sec/M_method_old.tex <==
% For 3D motion forecasting, the apparent motion in the static background is primarily caused by the camera motion, also known as ego-motion \cite{zhou2017unsupervised, schmied2023r3d3}. Ego-motion forecasting is crucial as it underpins the ability to predict future states of the scene from the perspective of a moving observer. The challenge here lies in accurately modeling the camera's movement in 3D space, which influences all observed elements in the scene. Failure to precisely forecast ego-motion can lead to significant inaccuracies in the predicted scene dynamics, as even minor deviations in camera trajectory prediction can cause large deviations in the visual outcome. 

% For 3D scene forecasting, the apparent motion in the static background is primarily due to camera motion (\ie ego-motion) \cite{zhou2017unsupervised, schmied2023r3d3}. 
% \textcolor{red}{need more elaboration here: why ego-motion forecasting is critical, what is the challenge and how we address it. } 
% Hence, we design an ego-motion forecasting module accordingly. Additionally, to forecast the diverse motion scales exhibited by various foreground objects, we propose a multi-scale foreground forecasting module.  

\textbf{Method overview.} Our method aims to forecast a 3D scene into the future and view it from novel viewpoints. Initially, we predict dense depth maps for the input frames to accurately model the scene's geometry. Following this, we construct the 3D point cloud for each frame, where a 3D point contains a 3D location and a learnable appearance feature: (1) we generate 2D feature maps for from the input frame and an inpainted frame, which is specifically designed to address disocclusions. As a result, we obtain feature layers, denoted as $\mathcal{F}_{(t-1)}$ and $\mathcal{F}_{(t)}$, corresponding to each input frames. (2) These feature layers are then lifted into 3D space using corresponding depth values, generating point clouds $\mathcal{P}_{(t-1)}$ and $\mathcal{P}_{(t)}$. Later, we perform 3D motion forecasting using the obtained feature layers $\mathcal{F}_{(t-1)}$ and $\mathcal{F}_{(t)}$ as input. This forecasting allows us to displace the point clouds $\mathcal{P}_{(t-1)}$ and $\mathcal{P}_{(t)}$ according to the forecasted 3D motion flow, followed by separate 3D-to-2D splatting and rendering to obtain feature maps. Finally, we use a refinement network that takes these projected feature maps and decodes them to synthesize a novel view $\hat{I}'_{(t+1)}$ based on the target viewpoint. 


%\textcolor{red}{Since ViTA uses four frames (video information) for depth estimation, we can mention video-based depth estimation. If ViTA is only an option, consider to delay it to implementation details.} 


% We start by estimating 3D scene geometry using past frames $I_{(t-1)}$ and $I_{(t)}$ with an off-the-shelf depth prediction network.  We employ the publicly available ViTA network \cite{xian2023vita}, which ensures consistent depth predictions across frames, built upon MiDaS v2 \cite{ranftl2020towards}. ViTA's strength lies in maintaining depth consistency through optical flow correspondences. Consistent depth is critical as it prevents inaccuracies in 3D motion estimation, which, in turn, affects future frame synthesis. Formally, for the input frames, we compute the normalized depth maps, denoted as $D_{(t-1)}$ and $D_{(t)}$, where $D_{i} \in [0, 1]^{H \times W \times 3}$.  
\vspace{-2pt}
\subsubsection{Two-layer scene decomposition.} A major challenge in synthesizing photorealistic future frames is handling disocclusions caused by motion parallax in novel views and object motion.  Many 3D photography methods \cite{shih20203d, li20233d, jampani2021slide, wang20223d} employ depth-based layering \cite{li2021mine} to address disocclusions during view changes. Despite efficient treatment, they struggle with disocclusions resulted from various object motions within each depth layer. This challenge is further compounded when foreground objects move, leaving ``holes" behind in the background that disrupt the visual continuity and realism of the synthesized images.

To address this, our approach describes the scene into two distinctive layers: background (BG) {\bf inpaint} and original (ORG) (input frame with both background and foreground objects). The inpaint layer is formed by inpainting the ``holes" left by the foreground elements. 
In this way, we can ensure that, despite the disocclusions, content is present behind foreground objects. 
The inpaint layer mainly captures static elements, whereas the ORG layer encompasses all aspects of the scene. By utilizing a segmentation model such as DeepLabv3 \cite{chen2018encoder}, we differentiate BG from ORG across both input frames, creating distinct layered images $\mathcal{L}_{(t-1)}$ and $\mathcal{L}_{(t)}$. {\bf adding static categories}
Each layered image, denoted as $\mathcal{L}_{i}$, comprises a set of paired RGB color and depth images for both the inpaint layer $\{ \mathbf{C}_{i}^{BG}, \mathbf{D}_{i}^{BG} \}$ and original layer $\{ \mathbf{C}_{i}^{ORG}, \mathbf{D}_{i}^{ORG} \}$, alongside the background binary mask $\mathbf{M}_{i}$. 

% where  with paired RGB and depth images for both layers ${ \mathbf{C}{i}^{BG}, \mathbf{D}{i}^{ORG} }$, alongside a binary mask $\mathbf{M}_{i}$.. The BG layer is identified through the scene's static components. In contrast, the ORG layer encompasses the entire original scene, including both static and dynamic elements.  This strategy leverages a segmentation model \cite{chen2018encoder} to create a binary mask, effectively differentiating the BG layer from the ORG scene.  This segmentation process is systematically applied to consecutive input frames, resulting in distinct layers for each frame: $\mathcal{L}_{(t-1)}$ and $\mathcal{L}_{(t)}$. Each $\mathcal{L}_{i}$ comprises a set of paired RGB color and depth images for both the foreground $\{ \mathbf{C}_{i}^{BG}, \mathbf{D}_{i}^{ORG} \}$ and background $\{ \mathbf{C}_{i}^{BG}, \mathbf{D}_{i}^{ORG} \}$, alongside the background binary mask $\mathbf{M}_{i}$. Here, $\mathbf{C}^{l}$, $\mathbf{D}^{l}$, and $\mathbf{M}$ respectively represent the RGB color image, depth image, and background binary mask.

\subsubsection{Inpainting.} Subsequently, we inpaint occluded regions in the background layer using RGBD inpainting techniques such as 3D Photo \cite{shih20203d}, ensuring content is present behind foreground objects during disocclusions. 

% \subsubsection{Feature Extraction.} To enhance rendering quality and minimize artifacts of the forecasted future frames, we utilize a 2D feature extraction network $\phi(.)$, to process each image $\mathbf{C}^{l}$ {\bf use previous annotations} in BG and ORG layers. This process yields 2D feature maps, represented as $\mathbf{F}^{l}=\phi(\mathbf{C}^{l})$. Consequently, we organize these maps into feature layers, denoted by $\mathcal{F}_{i}$, which comprise of background features $\{ \mathbf{F}_{i}^{BG}, \mathbf{D}_{i}^{BG} \}$ and original features $\{ \mathbf{F}_{i}^{ORG}, \mathbf{D}_{i}^{ORG} \}$, along with the background binary mask $\mathbf{M}_{i}$.

==> sec/Y_tmp.tex <==
\newpage

$\mathbf{F}^{BG}$\\ \\

$\mathbf{F}^{ORG}$ \\ \\


$\mathbf{M}$ \\ \\

$\mathcal{F}_{i}$ \\ \\

$\mathcal{F}$ \\ \\

$\mathcal{F}_{(t-1)}$ \\ \\

$\mathcal{F}_{(t)}$ \\ \\

$\mathbf{F}_{(t-1)}$ \\ \\

$\mathbf{F}_{(t)}$ \\ \\

$\mathbf{F}_{(i)}$ \\ \\

$\mathcal{F}_{(t)}^{ORG}$ \\ \\


$\mathcal{F}_{(t-1)}^{ORG}$ \\ \\


$\mathbf{U}^{0}_{(t+1)}$ \\ \\


$\mathcal{F}_{(t)}^{\overline{\text{BG}}}$\\\\


$\mathbf{F}_{(t-1)}^{\overline{\text{BG}}}$\\\\


$\mathbf{F}_{(t)}^{\overline{\text{BG}}}$\\\\


$\mathbf{F}^{\overline{\text{BG}}}$\\\\

$\mathbf{F}$\\\\

$\mathbf{D}^{\overline{\text{BG}}}$\\\\

$\mathbf{D}$ \\ \\

$\mathbf{D}_{(t)}^{\overline{\text{BG}}}$\\\\


$\mathbf{D}_{(t-1)}^{\overline{\text{BG}}}$\\\\


$\mathbf{M}_{(t-1)}$\\\\

$\mathbf{M}_{(t)}$\\\\


$\mathbf{D}_{(t)}$\\\\


$\mathbf{D}_{(t-1)}$\\\\


$\mathbf{F}_{(t)}$\\\\


$\mathbf{F}_{(t-1)}$\\\\


$\mathbf{U}_{(t+1)}^{0}$\\\\

$\mathbf{U}_{(t+1)}^{L}$\\\\

$\mathcal{P}$ \\ \\

$\mathcal{F}^{\overline{\text{BG}}}$\\\\

$\mathbf{U}_{(t+1)}^{(i-1)}$\\\\


$\mathbf{U}_{(t+1)}^{(i)}$\\\\


${S}^{(i)}$\\\\

$\mathcal{T}_{(t-1) \rightarrow (t+1)}$\\\\


$\mathcal{T}_{(t) \rightarrow (t+1)}$\\\\
